Analysis and Design of Vehicle Platooning Operations on Mixed-Traffic Highways

Platooning of connected and autonomous vehicles (CAVs) has a significant potential for throughput improvement. However, the interaction between CAVs and non-CAVs may limit the practically attainable improvement due to platooning. To better understand and address this limitation, we introduce a new fluid model of mixed-autonomy traffic flow and use this model to analyze and design platoon coordination strategies. We propose tandem-link fluid model that considers randomly arriving platoons sharing highway capacity with non-CAVs. We derive verifiable conditions for stability of the fluid model by analyzing an underlying M/D/1 queuing process and establishing a Foster-Lyapunov drift condition for the fluid model. These stability conditions enable a quantitative analysis of highway throughput under various scenarios. The model is useful for designing platoon coordination strategies that maximize throughput and minimize delay. Such coordination strategies are provably optimal in the fluid model and are practically relevant. We also validate our results using standard macroscopic (cell transmission model, CTM) and microscopic (Simulation for Urban Mobility, SUMO) simulation models.

==> Texts/6_Biography.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./Images/Fig_Jin2.jpg}}]{Li Jin}
is an Assistant Professor at the New York University Tandon School of Engineering.
He received B.Eng. degree in Mechanical Engineering from Shanghai Jiao Tong University in 2011, M.S. degree in Mechanical Engineering from Purdue University in 2012, and Ph.D. degree in Transportation from the Massachusetts Institute of Technology in 2018.
He was also a visiting scholar at the University of Erlangen-Nuremberg in 2016.
His background is stochastic processes, dynamic control, and optimization.
His research focuses on developing resilient control algorithms for cyber-physical systems with guarantees of efficiency in nominal settings, robustness against random perturbations, and survivability under strategic disruptions.
%The theoretical foundation of his work include stochastic process and control theory. 
Specific applications of his work include connected and autonomous vehicles, automatic traffic control, air transportation, and gas network.
% He is a recipient of the Ho-Ching and Hang-Ching Fund Award and Schoettler Scholarship Fund.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./Images/Fig_Cicic.jpg}}]{Mladen \v Ci\v ci\'c} received his M.Sc. degree in automatic control from the School of Electrical Engineering, University of Belgrade, in 2015. He is pursuing the Ph.D degree at the Department of Automatic Control, KTH Royal Institute of Technology. He is a member of Marie Sk{\l}odowska Curie oCPS ITN and an affiliated Wallenberg AI, Autonomous Systems and Software Program (WASP) student. He was also a visiting scholar at the C2SMART University Transportation Center in the New York University Tandon School of Engineering in 2019. His research interests include traffic control using mixed traffic models. 
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./Images/Fig_Johansson}}]{Karl H. Johansson} is Professor at the School of Electrical Engineering and Computer Science, KTH Royal Institute of Technology, Sweden. He received MSc and PhD degrees from Lund University. He has held visiting positions at UC Berkeley, Caltech, NTU, HKUST Institute of Advanced Studies, and NTNU. His research interests are in networked control systems, cyber-physical systems, and applications in transportation, energy, and automation. He is a member of the Swedish Research Council's Scientific Council for Natural Sciences and Engineering Sciences. He has served on the IEEE Control Systems Society Board of Governors, the IFAC Executive Board, and is currently Vice-President of the European Control Association Council. He has received several best paper awards and other distinctions from IEEE, IFAC, and ACM. He has been awarded Distinguished Professor with the Swedish Research Council and Wallenberg Scholar with the Knut and Alice Wallenberg Foundation. He has received the Future Research Leader Award from the Swedish Foundation for Strategic Research and the triennial Young Author Prize from IFAC. He is Fellow of the IEEE and the Royal Swedish Academy of Engineering Sciences, and he is IEEE Control Systems Society Distinguished Lecturer.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./Images/Fig_Amin}}]{Saurabh Amin} is Robert N. Noyce Career Development Associate Professor in the Department of Civil and Environmental Engineering and a core faculty member in the Laboratory of Information and Decision Systems (LIDS), Massachusetts Institute of Technology. He received his Ph.D. in Systems Engineering from the University of California, Berkeley in 2011. His research focuses on the design and implementation of high confidence network control algorithms for infrastructure systems.
He works on robust diagnostics and control problems that involve using networked systems to facilitate the monitoring and control of large-scale critical infrastructures, including transportation, water, and energy distribution systems. 
He also studies the effect of security attacks and random faults on the survivability of networked systems, and designs incentive-compatible control mechanisms to reduce network risks. 
He is a recipient of NSF CAREER and Google Faculty Research awards. 
\end{IEEEbiography}


